Value of Assistance for Grasping

In multiple realistic settings, a robot is tasked with grasping an object without knowing its exact pose and relies on a probabilistic estimation of the pose to decide how to attempt the grasp. We support settings in which it is possible to provide the robot with an observation of the object before a grasp is attempted but this possibility is limited and there is a need to decide which sensing action would be most beneficial. We support this decision by offering a novel Value of Assistance (VOA) measure for assessing the expected effect a specific observation will have on the robot's ability to complete its task. We evaluate our suggested measure in simulated and real-world collaborative grasping settings.

==> backup/extensions.tex <==
\begin{itemize}
    \item a single observation that affects multiple agents
    \item Account for noisy sensor
    \item observation has irrelevant information
\end{itemize}

==> backup/tables.tex <==
\begin{table}
\begin{adjustbox}{angle=0}
\begin{tabular}{|cc|cccc|cc|}
\specialrule{.1em}{0em}{0em} % Set top rule width
\multirow{2}{*}{}
& & \multicolumn{4}{c|}{$\objPose_1$} & &  \\
\specialrule{.1em}{.1em}{.1em} % Set midrule width
&  & $\graspConfigMax$ & score & pred. $ \graspConfigMax$ & pred. score & \VOA & \EVD \\
\specialrule{.1em}{.1em}{.2em} % Set midrule width
& true &          0 & 0.86 & - & - & - & - \\
\hline
& $\helperConfig$ & & & & & & \\
& $\emptyset$ &    3 & 0.57 & - & - & - &  - \\
\specialrule{.1em}{0em}{0em} % Set midrule width
\multirow{4}{*}{$\beliefUpdateFunc_1$}  
& $I$ &  0 & 0.86 & 0 & 0.86 & 0.27 & 0.27 \\
& $II$ &  0 & 0.86 &  0 & 0.86 & 0.27 & 0.27 \\
& $III$ &  0 & 0.86 & 0 & 0.86 & 0.27 & 0.27 \\
& $IV$ &  0 & 0.86 & 0 & 0.86 & 0.27 & 0.27 \\
\specialrule{.1em}{0em}{0em} % Set midrule width
\multirow{4}{*}{$\beliefUpdateFunc_2$}  
& $I$ & 0 & 0.80 & 0 & 0.80 & {\bf 0.21} & {\bf 0.21} \\
& $II$ & 0 & 0.73 & 0 & 0.73 & 0.19 & 0.19 \\
& $III$ & 0 & 0.68 & 0 & 0.68 & 0.19 & 0.18 \\
& $IV$ & 0 & 0.77 & 0 & 0.77 & 0.2 & 0.19 \\
\specialrule{.1em}{0em}{0em} % Set midrule width
\multirow{4}{*}{$\beliefUpdateFunc_3$} 
& $I$ & 0 & 0.85 & 0 & 0.85 & {\bf 0.25} & {\bf 0.25} \\
& $II$ & 0 & 0.81 & 0 & 0.80 & 0.23 & 0.23 \\
& $III$ & 0 & 0.63 & 0 & 0.63 & 0.2 & 0.2 \\
& $IV$ & 0 & 0.85 & 0 & 0.85 & 0.24 & 0.24 \\
\specialrule{.2em}{0em}{0em} % Set bottom rule width
& $\emptyset$ &    0 & 0.56 & - & - & - &  - \\
\specialrule{.1em}{0em}{0em}
\multirow{6}{*}{$\beliefUpdateFunc_4$} 
& $I$ &  0 & 0.78 & 0 & 0.82 & {\bf 0.14} & {\bf 0.23} \\
& $II$ &  0 & 0.68 &  0 & 0.81 & 0.12 & 0.12 \\
& $III$ &  0 & 0.71 & 0 & 0.76 & 0.11 & 0.11 \\
& $IV$ &  0 & 0.74 & 0 & 0.79 & 0.12 & 0.16 \\
& $V$ & 0 & 0.58 & 0 & 0.79 & 0.12 & 0.01 \\
& $VI$ & 0 & 0.64 & 0 & 0.80 & 0.13 & 0.06 \\
\specialrule{.1em}{0em}{0em} % Set midrule width
\multirow{6}{*}{$\beliefUpdateFunc_5$}  
& $I$ & 0 & 0.61 & 0 & 0.61 & 0.02 & {\bf 0.04} \\
& $II$ & 0 & 0.59 & 0 & 0.61 & 0.02 & 0.02 \\
& $III$ & 0 & 0.60 & 0 & 0.60 & 0.01 & 0.02 \\
& $IV$ & 0 & 0.60 & 0 & 0.6 & 0.02 & 0.02 \\
& $V$ & 0 & 0.55 & 0 & 0.61 & 0.02 & -0.01 \\
& $VI$ & 0 & 0.58 & 0 & 0.62 & {\bf 0.03} & 0.01 \\
\specialrule{.1em}{0em}{0em} % Set midrule width
\multirow{6}{*}{$\beliefUpdateFunc_6$}
& $I$ & 0 & 0.73 & 0 & 0.86 & {\bf 0.26} & 0.21 \\
& $II$ & 3 & 0.55 & 0 & 0.85 & 0.24 & 0.04 \\
& $III$ & 3 & 0.66 & 0 & 0.85 & 0.25 & 0.13 \\
& $IV$ & 2 & 0.77 & 0 & 0.84 & 0.22 & 0.17 \\
& $V$ & 2 & 0.60 & 0 & 0.86 & {\bf 0.26} & {\bf 0.24} \\
& $VI$ & 0 & 0.87 & 0 & 0.86 & {\bf 0.26} & 0.15 \\
\specialrule{.2em}{0em}{0em} % Set bottom rule width

\end{tabular}
\end{adjustbox}

\caption{HOLDER lab results per belief update function}
\label{tab:voa-flask}

\end{table}

\begin{table}[h]
\label{table:obs_pred_eval}
    \centering
    \begin{tabular}{|c|c|c||c|c|c|}
        \hline  % Horizontal line
        \multicolumn{3}{|c||}{\textbf{Lidar}} & \multicolumn{3}{c|}{\textbf{Depth Image}} \\
        \hline
        $\helperConfig$ & Avg. Err. & Min. Err. & $\helperConfig$ & Avg. IoU & Max IoU  \\
        \hline
        $I$ & 1.6 & 0.7 & $I$ & 0.6 & 0.8\\  
        $II$ & 3.9 & 0.7 & $II$ & 0.5 & 0.7\\  
        $III$ & 0.8 & 0.5 & $III$ & 0.6 & 0.7 \\
        $IV$ & 3.0 & 0.6 & $IV$ & 0.6 & 0.7 \\ 
        - & - & - & $V$ & 0.4 & 0.6 \\ 
        - & - & - & $VI$ & 0.3 & 0.5\\ 
        \hline
    \end{tabular}
    \caption{Observation prediction evaluation for  HOLDER}
    \label{tab:obs_pred_eval}
\end{table}


==> backup/voadef.tex <==
We let $\beliefUpdateFunc_{\actorSymbol}$ and $\beliefUpdateFunc_{\helperSymbol}$ represent the belief update functions of the \actor~and~\helper, respectively. Accordingly, 
$\actorBelief^{\observation,\beliefUpdateFunc_{\actorSymbol}}$ and $\helperBelief^{\observation,\beliefUpdateFunc_{\helperSymbol}}$ represent the \actor's and \helper's belief after receiving observation $\observation$ and updating their belief, i.e., $\actorBelief^{\observation,\beliefUpdateFunc} = \beliefUpdateFunc_{\actorSymbol} (\poseBeliefActor, \observation)$ and $\helperBelief^{\observation,\beliefUpdateFunc} = \beliefUpdateFunc_{\helperSymbol} (\poseBeliefHelper, \observation)$.
A key element in \VOA~computation is the difference between the expected score
$\graspScoreExpectation(\graspConfigMax(\actorBelief^{\observation,\beliefUpdateFunc_{\actorSymbol}}),\poseBeliefHelper^{\observation, \beliefUpdateFunc_{\helperSymbol}})
$ of the maximal grasp after receiving an observation $\observation$ and without receiving it, i.e., 
$\graspScoreFunc(\graspConfigMax(\actorBelief),\poseBeliefHelper)$. 


\begin{sloppypar}

\begin{definition}[Value of Assistance (\VOA) for Grasping]
Given \actor~belief $\poseBeliefActor \in \allPoseBeliefs$, \helper~belief $\poseBeliefHelper \in \allPoseBeliefs$, a perceived sensor function $\observationPerceivedProbability_{\helperSymbol}$, sensor configuration $\helperConfig \in \helperConfigs$ and belief update functions of the \actor~and~\helper~$\beliefUpdateFunc_{\actorSymbol}$ and $\beliefUpdateFunc_{\helperSymbol}$,  
% \begin{equation}
\begin{align}
\VOAFunc_{\assistanceAction}&(\helperBelief,\actorBelief)  \eqdef\\
& \mathbb{E}_{\objPose \sim \helperBelief}
\left[
\mathbb{E}_{\observation \sim \observationPerceivedProbability_{\helperSymbol}\left({\observation \vert \objPose, \helperConfig }\right)}
\left[
\graspScoreExpectation(\graspConfigMax(\actorBelief^{\observation,\beliefUpdateFunc_{\actorSymbol}}),\poseBeliefHelper^{\observation, \beliefUpdateFunc_{\helperSymbol}})
\right]
- \graspScoreExpectation(\graspConfigMax(\actorBelief),\poseBeliefHelper))\right]
\end{align}
% \end{equation}
\end{definition}
\end{sloppypar}

Since \VOA~estimation is done by the \helper, observation $\observation$ is extracted from its perceived observation probability $\observationPerceivedProbability_{\helperSymbol}$. In contrast, the \actor's belief update using Equation \ref{eq:belief update} is based on its own perceived observation probability $\observationPerceivedProbability_{\actorSymbol}$.

---------------


==> content/background.tex <==
\section{Background}\label{sec:bg}
\subsection{Grasping}
\subsection{Modeling Grasping Uncertainty}
A {\em belief} $\belief: \states \mapsto [0,1]$ is 

\subsection{\VOA}

XXX define \emph{Value of Assistance} (\VOA) as the difference between the expected cost of following a planned path and the expected cost of following the same path, but when receiving assistance.


==> content/backup.tex <==


---------------------------

observation space = $[o_1, o_2, o_3]$

state space = $[s_1, s_2, s_3, s_4]$

given that the observation is $o_1$

$$p(o_1|s_1)= \frac{p(s_1|o_1)\cdotp(o_1)}
{p(s_1)}$$


$p(o_2|s_1)$
$p(o_3|s_1)$

$p(o_1|s_2)$
$p(o_2|s_2)$
$p(o_3|s_2)$

$p(o_1|s_3)$
$p(o_2|s_3)$
$p(o_3|s_3)$

$p(o_1|s_4)$
$p(o_2|s_4)$
$p(o_3|s_4)$

Given that the object is at position $\objPose$
$\obsDisScore(o_1,o_1)$
$\obsDisScore(o_1,o_2)$
$\obsDisScore(o_1,o_3)$
$\obsDisScore(o_1,o_4)$


$$score(s_1|o_1)= 
\frac{\obsDisScore(o_1,o_1)}
{p(s_1)}$$


-----------\\

$H = - \sum_{i=1}^{n}score_i\cdot \log_2(score_i)$

------------------







--------------------




$\poseBelief_{\objPose}(\objPose')$ is \begin{equation}\label{eq:beliefUdpateRMSD}
\poseBelief_{\objPose}(\objPose') = \frac{\poseBelief(\objPose)\left(\rmsd(\estimatedSensorFunc(\objPose, \sensingAction), \estimatedSensorFunc(\objPose', \sensingAction))+\varepsilon\right)^{-1}}{\mathbb{E}_{\objPose'' \sim \poseBelief}\left[\left(\rmsd(\estimatedSensorFunc(\objPose'', \sensingAction), \estimatedSensorFunc(\objPose, \sensingAction))+\varepsilon\right)^{-1}\right]}
\end{equation}

For simplicity denote $r_{\sensingAction}(\objPose, \objPose') = \left(\rmsd(\estimatedSensorFunc(\objPose, \sensingAction), \estimatedSensorFunc(\objPose', \sensingAction))+\varepsilon\right)^{-1}$

Thus \begin{equation}\label{eq:beliefUdpateRMSD}
\poseBelief_{\objPose'}(\objPose) = \frac{\poseBelief(\objPose)r_{\sensingAction}(\objPose, \objPose')}{\mathbb{E}_{\objPose'' \sim \poseBelief}\left[r_{\sensingAction}(\objPose'', \objPose')\right]}
\end{equation}

If we expand the denominator:

Thus \begin{equation}\label{eq:beliefUdpateRMSD}
\poseBelief_{\objPose'}(\objPose) = \frac{\poseBelief(\objPose)r_{\sensingAction}(\objPose, \objPose')}{\poseBelief(\objPose)r_{\sensingAction}(\objPose_0, \objPose') + ... + \poseBelief(\objPose)r_{\sensingAction}(\objPose, \objPose') + ... + \poseBelief(\objPose)r_{\sensingAction}(\objPose_{\|\allObjStablePoses\|}, \objPose')}
\end{equation}

Now if we sum for all entries we will get 1 (each element in the sum has the same denominator):
$ \sum_{\objPose \in \poseBelief}\poseBelief_{\objPose'}(\objPose) = $
\begin{equation}
     = \frac{\poseBelief(\objPose)r_{\sensingAction}(\objPose_0, \objPose') + ... + \poseBelief(\objPose)r_{\sensingAction}(\objPose, \objPose') + ... + \poseBelief(\objPose)r_{\sensingAction}(\objPose_{\|\allObjStablePoses\|}, \objPose')}{\poseBelief(\objPose)r_{\sensingAction}(\objPose_0, \objPose') + ... + \poseBelief(\objPose)r_{\sensingAction}(\objPose, \objPose') + ... + \poseBelief(\objPose)r_{\sensingAction}(\objPose_{\|\allObjStablePoses\|}, \objPose')}
\end{equation}

For any similarity function $s_{\sensingAction}(\objPose_0, \objPose')$, we aim to achieve the following: $s_{\sensingAction}(\objPose_0, \objPose') \propto \poseBelief_{\objPose'}(\objPose)$, and $r_{\sensingAction}(\objPose_0, \objPose')$ achieves that.





$$
    \poseBelief\left({\observation \vert \objPose, \sensorConfig}\right) =
\left\lbrace{
\begin{array}{cc}
   \frac{1}{\eta}  & \estimatedSensorFunc\left({\objPose, \sensorConfig}\right) = \estimatedSensorFunc\left({\objPose_{i}, \sensorConfig}\right)\\
   0  & \estimatedSensorFunc\left({\objPose, \sensorConfig}\right) \neq \estimatedSensorFunc\left({\objPose_{i}, \sensorConfig}\right)
\end{array}
}\right.
$$

==> content/belief_update_sarah.tex <==
\section{Belief Update SARAH}


We define a distance metric between two observations 
% define distance function
\begin{definition}[Observation Similarity Metric]
Given two observations $\observation, \observation' \in \observations$, a {\em observation similarity metric} $\obsSimScore:\observations\times\observations\mapsto %\mathbb{R}_{\geq0}$
[0,1]$
associates a similarity score $\obsSimScore(\observation, \observation')$ between two observations.
\end{definition}




Here we assume that $\estimatedSensorFunc$ is deterministic and noiseless, such that the distance between two observations taken from the same sensor configurations (and the same sensing action) are the same (and the distance between them is 0). 

In this work, observations are 360 floats array where each entry is associated with a degree. The distance between two observations $\observation, \observation' \in \observations$ is computed based on the \rmsd~measure as follows:
\begin{equation}\rmsd (\observation, \observation') =  \sqrt{\frac{\sum_{i=0}^{n-1}(\observation[i] - \observation'[i])^2}{n}}
\end{equation}
where $n=360$ and $\observation[i]$ is the value at cell $i$.

\todo{decide if it is better to use predicated observation in formula 4}

\todo{change this to a vector subtraction formulation}

As a reminder, we are dealing here with expected observations that are generated by our observation prediction function such that $\estimatedSensorFunc$. 
$$\estimatedObservation_{\objPose,\sensingAction} = \estimatedSensorFunc\left({ \objPose, \sensingAction}\right)$$

Our observation similarity metric
is then
\begin{equation}\label{eq:obsScoree}
\obsSimScore(\estimatedObservation_{\objPose,\sensingAction}, \estimatedObservation_{\objPose',\sensingAction})= 1-\frac{\rmsd(\estimatedObservation_{\objPose,\sensingAction}, \estimatedObservation_{\objPose',\sensingAction})}{\sum_{\objPose'' \in \allObjStablePoses}\rmsd(\estimatedObservation_{\objPose,\sensingAction},\estimatedObservation_{\objPose'',\sensingAction} )}
\end{equation}

Our assumption here is that there is 
We assume that at least there is a pose that results an \rmsd~that is non zero.

Given Equation \ref{eq:obsScoree}, we can define a probability distribution as the weighted score of a pose given an observation

%\begin{equation}
%\probFunc(\objPose|\observation) =  
%\end{equation}
    


\sk{Find the advantage/informative value/entropy of the predicted observation given an object pose $\objPose$ and sensing action $\sensingAction$} 
%find a way to quantify how informative an observation is The observation that we get is
%$\observation_{\objPose,\sensingAction} = \estimatedSensorFunc\left({ \objPose, \sensingAction}\right)$
%The observation for object pose $\objPose'$ is
%$\observation_{\objPose',\sensingAction} = \estimatedSensorFunc\left({ \objPose', \sensingAction}\right)$

If the actual pose is $\objPose_i$.
The score of an observation is equivalent to how much it increases our certainty of each pose $\objPose_j$ where $j=\{0,1,...,i,...,|\allObjStablePoses|\}$.


% \begin{equation}\label{eq:obsScore}
% \obsScore(\objPose_j,\estimatedObservation_{\objPose_i,\sensingAction})= \frac{1-\obsDisScore(\estimatedObservation_{\objPose_i,\sensingAction}, \estimatedObservation_{\objPose_j,\sensingAction})}{\sum_{\objPose \in \allObjStablePoses}\left(1-\obsDisScore(\estimatedObservation_{\objPose_i,\sensingAction}, \estimatedObservation_{\objPose,\sensingAction})\right)}
% \end{equation}



Compute the belief update - how does the observation change my belief given my current belief

%compute the Baysian update


\begin{equation}\label{eq:beliefUpdate}
\poseBelief'_{\estimatedObservation}(\objPose) = \frac{P(\estimatedObservation|\objPose)\cdot\poseBelief(\objPose)}{P(\estimatedObservation)}  
\end{equation}

    

where $P(\estimatedObservation|\objPose) = \obsSimScore(\estimatedObservation, \estimatedObservation_{\objPose,\sensingAction})$ and $$P(\estimatedObservation) = \sum_{p'\in\allObjStablePoses}P(\estimatedObservation|\objPose')\cdot\poseBelief(\objPose')$$


We now perform the belief update - how does the observation change my belief given my current belief and given that the object is at pose $p_i$


 \begin{equation}\label{eq:beliefUdpate}
 \poseBeliefPerPose' = \beliefUpdateFunc\left({\poseBelief, \estimatedSensorFunc\left({ \objPose, \sensingAction}\right)}\right)= \beliefUpdateFunc\left({\poseBelief, \estimatedObservation_{\objPose,\sensingAction}}\right) 
\end{equation}

\begin{equation}\label{eq:beliefUdpate}
 \poseBeliefPerPose'(\pose_i) =  
 \poseBelief(\pose_i)\frac{
\obsSimScore(\estimatedObservation_{\objPose,\sensingAction}, \estimatedObservation_{\objPose_i,\sensingAction})}{\sigma_{\objPose\in \allObjStablePoses}
\end{equation}



==> content/grasp-voa-yuval.tex <==

\begin{figure}[t]
%\vspace{0.18cm}
\centering
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 2mm 4mm 6mm 4mm, clip, width=1\textwidth]{images/sensor_config_0.png}
\caption{}
\label{fig:example-obj-configs_a}
\end{subfigure}    %\hfil
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 2mm 4mm 6mm 4mm, clip, width=1\textwidth]{images/sensor_config_1.png}
\caption{}
\label{fig:example-obj-configs_b}
\end{subfigure}  
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 2mm 4mm 6mm 4mm, clip, width=1\textwidth]{images/sensor_config_2.png}
\caption{}
\label{fig:example-obj-configs_c}
\end{subfigure}    %\hfil
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 2mm 4mm 6mm 4mm, clip, width=1\textwidth]{images/sensor_config_3.png}
\caption{}
\label{fig:example-obj-configs_d}
\end{subfigure}

\caption{Example sensor configurations. Each column represents the RGB image [top] lidar reading [middle]  and depth image [bottom] for a sensor configuration-object pose pair.}
\label{fig:example-sense-configs1}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 0mm 25mm 0mm, clip, width=1\textwidth]{images/endstop_grasp_0.png}
\caption{}
\label{fig:example-grasp-configs_a}
\end{subfigure}
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 0mm 25mm 0mm, clip,width=1\textwidth]{images/endstop_grasp_1.png}
\caption{}
\label{fig:example-grasp-configs_b}
\end{subfigure}
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 0mm 25mm 0mm, clip,width=1\textwidth]{images/endstop_grasp_2.png}
\caption{}
\label{fig:example-grasp-configs_c}
\end{subfigure}
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 0mm 25mm 0mm, clip,width=1\textwidth]{images/endstop_grasp_3.png}
\caption{}
\label{fig:example-grasp-configs_d}
\end{subfigure}
\caption{Example grasp configurations from which the \actor~can attempt to grasp the object - each configuration is associated with a score, i.e., probability of success.}
\label{fig:example-grasp-configs}
\end{figure}


\begin{figure}[t]
\centering
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 5mm 25mm 5mm, clip, width=1\textwidth]{images/endstop_pose_0.png}
\caption{}
\label{fig:example-obj-configs_a}
\end{subfigure}    %\hfil
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 5mm 25mm 5mm, clip, width=1\textwidth]{images/endstop_pose_1.png}
\caption{}
\label{fig:example-obj-configs_b}
\end{subfigure}  
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 5mm 25mm 5mm, clip, width=1\textwidth]{images/endstop_pose_2.png}
\caption{}
\label{fig:example-obj-configs_c}
\end{subfigure}    %\hfil
\begin{subfigure}{0.1168\textwidth}
\centering
\includegraphics[trim = 25mm 5mm 25mm 5mm, clip, width=1\textwidth]{images/endstop_pose_3.png}
\caption{}
\label{fig:example-obj-configs_d}
\end{subfigure}    %\hfil
\caption{Example stable poses of the object.}
\label{fig:example-obj-configs}
\end{figure}

\section{Preliminaries} \label{sec: VOA}

Since we aim to support the grasping of an object that is assumed to be in a stable pose, we use a function that assigns a score to a grasping configuration - stable pose pair.
\begin{definition}[Grasp Score]
Given a set of object poses $\allObjStablePoses$ and  a set of grasp configurations $\graspConfigSet$, 
a {\em grasp score function} 
$\graspScoreFunc: \graspConfigSet \times \allObjStablePoses \mapsto [0,1]$
specifies the probability a \actor~applying grasp configuration $\graspConfig\in \graspConfigSet$ will successfully grasp an object at pose $\objPose \in \allObjStablePoses$,
i.e. 
$
\graspScoreFunc\left({\objPose, \graspConfig}\right) = P\left({ s \vert \objPose, \graspConfig}\right)
$, where $s$ is the event of a successful grasp. 
%associates each grasping configuration $\graspConfig \in \graspConfigSet$ to the probability of successfully grasping the object from that configuration when the object pose is $\objPose$.  
\end{definition}

The grasp score function may be evaluated analytically, by considering diverse factors such as contact area, closure force, object shape, and friction coefficient \cite{Murray1994AMI, DBLP:conf/icra/BicchiK00} or empirically, by using data-driven approaches such as \cite{mahler2017dex} where a deep learning model is trained to predict the quality of grasps based on depth images of the objects to be grasped.


%In our setting, the agent attempts to grasp an object for which the exact pose may not be known, perhaps since the pose is modeled as a stochastic process.

The \actor's choice of a grasp configuration relies on a {\em pose belief} which describes the agent's perceived likelihood of the object poses in the set of possible stable poses $\objStablePoses$.

\begin{definition}[Pose Belief]\label{def:poseBel}
%Given a set $\objStablePoses$ of possible (stable) object poses, 
A {\em pose belief} $\poseBelief: \objStablePoses \mapsto [0,1]$ is a probability distribution over $\objStablePoses$.
\end{definition}
%We note that the difference between the belief and the actual object pose probability distribution is that
The pose belief is affected by different factors, including the model of the object and its dynamics and collected sensory information. We formulate the initial belief after the object is dropped (Figure \ref{fig:example-setup}) using a joint probability model that captures the prior probability of stable poses, a von Mises PDF for the angle\cite{mardia2009directional}, and a multivariate normal distribution for the position on the plane. 
Formally, $\poseBelief(\objPose=(C, \theta, X, Y))=P(C)\cdot f(\theta;\mu_\theta,\kappa) \cdot f_{XY}(X,Y;\mu,\Sigma)$

where:\sk{where do we consider the dynamics of the fall?}
\begin{itemize}
    \item $P(C)$ is the probability of the category $C$, where $C$ is a discrete random variable representing the category of stable poses for a given object. The variable $C$ takes values from a finite set of predefined categories, each corresponding to a distinct stable pose of the object. For example, the adversarial object in our example has five distinct categories, corresponding to the sides with a large enough surface.  
    \item $f(\theta;\mu_\theta,\kappa)$ is the probability density function (PDF) of the von Mises \cite{mardia2009directional} distribution for the object's angle $\theta$, with mean direction $\mu_\theta$ and concentration parameter $\kappa$.
    \item $f_{XY}(X,Y;\mu,\Sigma)$ is the joint PDF of the multivariate normal distribution for position $(X,Y)$, with mean vector $\mu$ and covariance matrix $\Sigma$.
\end{itemize}

The \actor~uses its pose belief $\poseBelief$ and grasp score function $\graspScoreFunc$ to select a grasping configuration $\graspConfig\in \graspConfigSet$ from which to attempt to grasp the object.
A reasonable choice is to select a configuration that maximizes the \emph{expected grasp score}.

\begin{definition}[Expected Grasp Score] 
For grasp configuration $\graspConfig$ and pose belief $\poseBelief$, the {\em \expectedGraspScore} $\graspScoreExpectation(\graspConfig, \poseBelief)
=
\mathbb{E}_{\objPose \sim \poseBelief}[\graspScoreFunc\left({ \graspConfig, \objPose }\right)]$
is the weighted aggregated grasp score over the set of possible poses
A \emph{maximal grasp} $\graspConfigMax$ maximizes the expected grasp score, i.e.,
$\graspConfigMax(\poseBelief) = \argmax_{\graspConfig\in \graspConfigSet}{\graspScoreExpectation\left({\graspConfig, \poseBelief}\right)}$.
\end{definition}

In our setting, the \actor~receives an {\em observation} from the \helper~which corresponds to its readings from a specific sensor configuration $\helperConfig \in \helperConfigs$ and object pose $\objPose \in \allObjStablePoses$. %\sk{I want to remove sensing actions for now: We denote these interventions as {\em sensing actions} $\sensingActions$.Each sensor configuration emits an observation $\observation$ and may be associated with an environment-specific cost.}
%The set of possible sensing configurations  and sensing function induce an {\em observation space}.
Our formulation of the {\em observation space} $\observations$ is general and represents the set of readings that can be made for the sensor used in the considered setting. Here, we use two sensor types that may be available: a planar lidar sensor from which a reading is an array representing distances per angle $\mathbb{R}_{\geq 0}^{360}$ and a depth camera which emits a  
2D array $\mathbb{R}_{\geq 0}^{w \times h}$, where $w \times h$ are the image dimensions.

We consider obtaining an observation as a stochastic process as defined in \cite{lauri2022partially}. 

\begin{definition}[Observation Function]
\label{def:obsFunc} Given object pose $\objPose \in \allObjStablePoses$, sensor configuration $\helperConfig \in \helperConfigs$, and observation $\observation \in \observations$, a stochastic observation function $\sensorFunc\left({\observation,\objPose, \helperConfig}\right) = 
P\left({\observation \vert \objPose, \helperConfig }\right)$ 
provides the conditional probability of obtaining $\observation$ from $\helperConfig$ for $\objPose$.
\end{definition}
We note that the \actor~may not be aware of the actual observation probability distribution. Instead, it only has a \emph{perceived observation probability} $\observationPerceivedProbability\left({\observation \vert \objPose, \helperConfig}\right)$, based on a predefined, perhaps wrong,  probability distribution.
%A sensing action $\sensingAction \in \sensingActions$ is a random sampling of a single observation $\observation \in \allObservations$ given an observation probability distribution.

%We note that we support here a deterministic function, \sk{TODO: discuss its extension to probabilistic estimations.}

%Here, a set  given $\sensingActions$ of possible sensing actions are 

%such that for every   $\sensingAction(\poseBelief_{t}) = \poseBelief_{t+1}$.

%Our objective is to find the sensor configuration that offers the highest $\Utility$ after the intervention. 


%The \helper~maintains a pose belief $\poseBelief$ (Definition \ref{def:poseBel}).
When receiving an observation $\observation$, the \actor~updates its belief using its \emph{belief update function} which defines the effect an observation has on the pose belief.


\begin{definition}[Belief Update]
A belief update function \\
$\beliefUpdateFunc: \allPoseBeliefs \times \allObservations  \mapsto \allPoseBeliefs$ maps a given belief $\poseBelief\in \allPoseBeliefs$ and a given observation $\observation \in \allObservations$ to an updated belief.
\end{definition}

%As is common in the literature \todo{Insert citations here}, we assume the agent uses a Bayesian  filter for its implementation of $\beliefUpdateFunc$. 
%Accordingly, for every object pose $\objPose \in \objStablePoses$ and possible observation $\observation \in \allObservations$, the updated pose belief $\updatedPoseBelief\left({\objPose}\right)$ for a given pose $\objPose$ is given as


The literature is rich with approaches for belief update (e.g., \cite{thrun2005probabilistic,stachniss2005information,indelman2015planning,kurniawati2022partially}). We assume a Bayesian filter is used such that for any  observation $\observation \in \allObservations$, the updated pose belief $\poseBelief_{\observation}\left({\objPose}\right)$ for a given pose $\objPose \in \objStablePoses$ is given as
\begin{comment}
\begin{equation}
\label{eq:belief update}
\poseBelief_{\helperConfig}\left({\objPose}\right)
=
\dfrac{
\observationPerceivedProbability\left({\observation \vert \objPose, \helperConfig}\right)
\poseBelief\left({\objPose}\right)
}{
\Sigma_{\objPose' \in \objStablePoses}
\observationPerceivedProbability\left({\observation \vert \objPose', \helperConfig}\right) \poseBelief\left({\objPose'}\right)
},
\end{equation}
\end{comment}
\begin{equation}
\label{eq:belief update}
\poseBelief_{\observation,\helperConfig}\left({\objPose}\right)
=
\dfrac{
\observationPerceivedProbability\left({\observation \vert \objPose, \helperConfig}\right)
\poseBelief\left({\objPose}\right)
}{
\int_{\objPose' \in \objStablePoses}
\observationPerceivedProbability\left({\observation \vert \objPose', \helperConfig}\right) \poseBelief\left({\objPose'}\right)
d\objPose'
}
\end{equation}

\noindent where
$\poseBelief\left({\objPose}\right)$ is the estimated probability that $\objPose$ is the object pose prior to considering the new observation $\observation$.


\section{Value of Assistance (\VOA) for Grasping}

We offer ways to assess the effect sensing actions will have on the probability of successfully grasping an object.
%We formulate this as a two-agent setting with a {\em \actor} and a {\em \helper}. The \actor~is required to choose a configuration from which to attempt to grasp an object. While the \actor~cannot sense the object and only has some prior belief regarding the object's possible poses, it can receive a single sensor reading or {\em observation} from the \helper. We focus on assessing the effect a sensor reading will have on the \actor's choice of configuration from which to attempt the % single attempt at the grasp. This is aimed at supporting the selection of the sensing action that maximizes the probability of a successful grasp. 
%Specifically, given the \actor~current belief regarding  the object's pose and a set of possible grasping actions, we seek a measure that predicts the effect each sensing action will have on the probability of successfully grasping the object. 
We formulate this as a two-agent collaborative grasping setting in which an {\em \actor} is tasked with grasping an object for which the exact pose is not known.
The \actor~needs to choose a configuration from which to attempt a grasp based on its {\em pose belief}, a distribution over the object's possible stable poses. The second agent, the {\em\helper,} can move to a specific configuration within its workspace to collect an observation from its sensor and share it with the \actor. %However, since such sensing actions may be costly and limited, there is a need for efficient ways to asses which observation would be most beneficial. %for the grasping task. 

We note that we use a two-agent model since it clearly distinguishes between the grasping and sensing capabilities.
Depending on the application, this model can be used to support an active perception setting in which a single agent needs to choose whether to perform a manipulation or sensing action if it is has the capability to do both.
%Also, while our focus here is on maximize the next grasp attempt, our measure is relevant both to settings in which the agent has only one grasp attempt (e.g. since the object is moving away) and to settings in which these measures are used for long-term planning (e.g., assessing the outcome of sensing actions within a POMDP).  


While the exact pose of the object is not known, its model is given and it is assumed to be at a stable pose (see Figure \ref{fig:example-obj-configs}). 
The \actor~needs to choose a feasible {\em \graspConfiguration} $\graspConfig$ from a set of possible configurations  
$\graspConfigSet$ from which a grasp will be attempted (see Figure \ref{fig:example-grasp-configs}) based on its pose belief $\poseBeliefActor$ and grasp score function $\graspScoreFunc$.
%associates each \graspConfiguration~stable pose pair with a score, representing the probability of successfully grasping the object from that configuration.
%However, . Formally, we assume the object pose $\objStablePose$ is modeled as a pose belief as defined above. \sk{within some known distribution of stable poses $\objStablePoses$.}  %While it can move to any valid grasp configuration in $\graspConfigSet$,  it cannot acquire new information about the object on its own before it attempts the grasp. The \actor~chooses a {\em grasp configuration} %for which the probability of success is known or can be estimated.

The \helper~can choose a single {\em sensor configuration} $\helperConfig$ from a set of possible configurations $\allHelperConfigs$ from which to capture an {\em observation}. 
Each possible sensor configurations offers a different point of view of the object and a potentially different effect on the
\actor's
pose belief and on the probability of a successful grasp (see Figure \ref{fig:example-sense-configs1}). 



%Dexterous space:
%$$ D=\{p=(x,y,z,R_x,R_y, R_z) | \exists q\in\mathbb(C),FK(q)=p\} $$
%where $\mathcal(C)$ is the configuration space and $FK$ is the forward kinematics function.

%It has a valid plan in free-space to each of these configurations. 

% that is transmitted to the \actor. 
%which it knows the shape of the object, it has a belief over the agent's positing. 
%\todo{specify assumptions}




We aim to assess Value of Assistance (\VOA) for grasping as the expected benefit an assistive action, in the form of an observation performed by the \helper, will have on the probability of a successful grasp by the \actor. %Accordingly,{\em Value of Assistance} (\VOA) caputres the difference between the highest expected grasp score before and after receiving an observation. 
Our perspective is that of the  \helper~and its decision of which sensing action to perform. Accordingly, we need a way to estimate beforehand the effect an expected observation will have on the \actor's belief and on its choice of configuration from which to attempt the grasp. 
%is the attempt to assess the effect an observation will have on the \actor's belief. 
%%A key to computing \VOA~is the ability to assess the perceived predicted observation probability,
%For this, there is a need to predict the observation that will be emitted when performing a sensing action. 
%In order to determine which sensing %action would be most beneficial, 
%We therefore define an 

\yuval{----moved from preliminaries and edited: (maybe move more forward?)}
\subsection{Prediction of the Updated Belief}
When the observation function $\sensorFunc$ is described as a stochastic process as in defenition \ref{def:obsFunc}, the probabilities can be used for directly describing $\observationPerceivedProbability$, and equation \ref{eq:belief update} can be used for belief update.

In some cases, $\sensorFunc$ can be deterministic. in those cases, instead of representing conditioned distribution of an observation given pose and helping action, it can map from a pose and a helping action directly to an observation: $\sensorFunc(\pose, \helperConfig) = \observation$.
In order to construct $\observationPerceivedProbability$ for a deterministic observation function, we use: an \emph{Observation Prediction Function} $\estimatedSensorFunc: \allObjStablePoses \times \helperConfigs \mapsto \allObservations$ that is predefined, and maps object pose and a sensor configuration to an estimated observation. In addition we have to define a  similarity score $\obsSimScore:\observations\times\observations\mapsto [0,1]$ between observation pairs $\observation$ and $\observation'$. The similarity metric and the predicted observation function, can be used to compose a valid distribution function for $\observationPerceivedProbability$ as follows:

\begin{equation}
    \observationPerceivedProbability(\observation|\pose, \helperConfig) = \frac{\obsSimScore(\estimatedSensorFunc(\objPose,\helperConfig), o)}{\int_{\objPose' \in \objStablePoses} \obsSimScore(\estimatedSensorFunc(\objPose',\helperConfig), o) d\objPose'}
\end{equation}

The following discussion presents three ways to implement $\obsSimScore$ but we note that our framework is not restricted to these methods. %Rather, we use them to demonstrate the variety of possible approaches to approximate the actual, unknown, observation probability.
The first measure deterministically decides whether two observations $\observation$ and $\observation'$ are equivalent, i.e.,  $ \observation \equiv \observation'$. We note that such a measure does not constrain the sensor to be deterministic but instead imposes a deterministic rule for deciding whether two observations are considered equivalent, e.g., if the difference between their values is within some bound. 

A second option is to use any arbitrary similarity metric as long as it simulates a probability in the sense that the Kolmogorov axioms \cite{Kolmogorov1933} are met when comparing one observation with the simulated probability distribution's mean.
For example, to assess structural similarity between depth image pairs $\observation$ and $\observation'$, we applied the Structural Similarity Index (SSIM) \cite{wang2004image} across localized windows, using the formula: $$\text{SSIM}(x, y) = \frac{(2\mu_x\mu_y + c_1)(2\sigma_{xy} + c_2)}{(\mu_x^2 + \mu_y^2 + c_1)(\sigma_x^2 + \sigma_y^2 + c_2)}
$$

where $x$ and $y$ are windowed segments within $\observation$ and $\observation'$, respectively. 
In this formula:
\begin{itemize}
    \item $\mu_x$ and $\mu_y$  are the average pixel values of windows $x$ and $y$, respectively.
    \item $\sigma_{x}^2$ and $\sigma_{y}^2$ are the variances of windows $x$ and $y$.
    \item $\sigma_{xy}$ is the covariance between windows $x$ and $y$.
    \item $c_1$ and $c_2$ are small constants to stabilize the division.
\end{itemize}
This method captures local structural patterns by averaging SSIM scores over all windows, providing a nuanced similarity measure that highlights spatial consistencies vital for analyzing depth images. This window-based SSIM calculation allowed for a detailed structural comparison, enriching our insights into the represented 3D scene's geometry.


As a third option, uncertainty is approximated using a compact parametric model, e.g., a Gaussian distribution, \todo{Mohamad - formulate as similarity score}.

Examples of these methods of approximating the observation probability are given in our empirical evaluation in Section \ref{sec: Empirical Evaluation}.

\yuval{-------end of part that moved from preliminaries}

% A key to computing \VOA~is
% an {\em observation prediction function}, that generates a synthetic observation that is predicted to be emitted if a sensing action is performed.
% \begin{definition}[Observation Prediction Function]\label{def:obsprediction}
% Given $\objPose \in \allObjStablePoses$ and $\helperConfig \in \helperConfigs$,
% {\em observation prediction function},
% $\estimatedSensorFunc: \allObjStablePoses \times \helperConfigs \mapsto \allObservations$, maps an object pose $\objPose\in \allObjStablePoses$ and a sensor configuration $\helperConfig \in \helperConfigs$      
% to an estimated observation $\estimatedObservation \in \allObservations$, i.e.
% $
% \estimatedObservation_{\objPose, \helperConfig}
% =
% \estimatedSensorFunc \left({\objPose, \helperConfig}\right).
% $
% \end{definition}

Note that the observation prediction function  
%$\observationPerceivedProbability\left({ \estimatedSensorFunc\left({\objPose', \helperConfig}\right) \vert \objPose, \helperConfig}\right)$. 
is equivalent to a deterministic sensing function, as defined in Definition \ref{def:obsFunc}.
%The discussion in Section \ref{sec:poseBelief} presents three different possible methods that can be used to assess the perceived observation probability by replacing observation $\observation$ with the predicated observation 
%\estimatedObservation_{\objPose, \helperConfig} = \estimatedSensorFunc \left({\objPose, \helperConfig}\right) $.
%We note that our method is general and supports any implementation of $\estimatedSensorFunc$.


Given a way to predict the observation a sensor will emit for each possible pose and sensing configuration and an understanding of how the \actor~will react to an observation by updating its pose belief, \VOA~captures the difference between the highest expected utility of the  \actor's belief before and after the intervention. 
Importantly, the \helper's belief may be different than that of the \actor,
as can the \actor's belief update function be.
We denote the \helper~and \actor's pose beliefs as $\poseBeliefHelper$ and $\poseBeliefActor$, respectively. The belief update function the \helper~associates with the \actor~is denoted by $\actorBeliefUpdate$. 
 %the probability of the \actor~successfully grasping the object from the chosen configuration.
 
% Notably, our focus here is not on estimating the effect an observation will have on the ability to identify the object's pose with high certainty such as was the focus in previous work \citet{}. Instead, we are interested in estimating the effect a sensing action will have on the choice of the grasp configuration to attempt and on the probability of the \actor~successfully grasping the object from the chosen configuration.

\begin{definition}[Value Difference For Grasping]
Given actor belief $\poseBeliefActor \in \allPoseBeliefs$, a helping action $\helperConfig \in \helperConfigs$, and a stable pose $\objStablePose$, Value difference is the mean difference between highest expected grasp score before and after receiving an observation:
\begin{equation}
\VDFunc_{\assistanceAction}(\objStablePose,\actorBelief) 
\eqdef 
\mathbb{E} \left[\graspScoreFunc(\graspConfigMax(\predictedActorBelief^{\assistanceAction}),\objPose)\right]
-
{\graspScoreFunc(\graspConfigMax(\actorBelief),\objPose)}
\end{equation}

\end{definition}

In the general case, the observation function can be stochastic, thus the grasp score after help is stochastic, and there is an expectation in the definition. In the case of a deterministic observation function, the expectation is not necessary:
\begin{equation}
\VDFunc_{\assistanceAction}(\objStablePose,\actorBelief) 
=
\graspScoreFunc(\graspConfigMax(\predictedActorBelief^{\assistanceAction}),\objPose)
-
{\graspScoreFunc(\graspConfigMax(\actorBelief),\objPose)}
\end{equation}

Ideally, the helper agent would be able to compute the value difference for to support it's decision about a helping action, but in practice, the pose is unknown, thus the actual value difference is intractable. Instead, the helper agent can estimate the value difference using it's belief $\poseBeliefHelper$. 

\begin{definition}[Value of Assistance (\VOA) for Grasping]
Given \actor~belief $\poseBeliefActor \in \allPoseBeliefs$, \helper~belief $\poseBeliefHelper \in \allPoseBeliefs$, and helping action $\helperConfig \in \helperConfigs$, Value of Assistance is the \textbf{estimated} difference between the highest expected grasp scores before and after receiving an observation, 

\begin{comment}
    
\begin{equation}\label{eq:generalVOAInf}
\VOAFunc_{\assistanceAction}(\helperBelief,\actorBelief) 
= 
\mathbb{E}_{\objPose \sim \poseBeliefActor}\left[\graspScoreFunc(\graspConfigMax(\actorBeliefUpdate(\poseBeliefActor,\estimatedObservation_{\objPose, \helperConfig})),\objPose)
-
\graspScoreFunc(\graspConfigMax(\poseBeliefActor),\objPose)
\right]
\end{equation}

\end{comment}
\begin{align}\label{eq:generalVOAInf1}
\VOAFunc_{\assistanceAction}(\helperBelief,\actorBelief) 
&\eqdef 
\mathbb{E}_{\objPose \sim \helperBelief}\left[\mathbb{E}[\graspScoreFunc(\graspConfigMax(\predictedActorBelief^{\assistanceAction}),\objPose)]
-
{\graspScoreFunc(\graspConfigMax(\actorBelief),\objPose)}\right] \\ 
&= \mathbb{E}_{\objPose \sim \helperBelief}\left[ 
\VDFunc(\objPose, \poseBeliefActor)
\right]
\end{align}

% where $\estimatedObservation_{\objPose, \helperConfig}$ is the estimated observation of object pose $\objPose$ from \helperConfiguration~$\helperConfig$ and  $\predictedActorBelief^{\assistanceAction} = \actorBeliefUpdate(\poseBeliefActor,\estimatedObservation_{\objPose, \helperConfig})$
% is the predicated \actor's belief after the observation is received. 
\begin{comment}
\begin{equation}
\label{eq:graspVOA}
\VOAFunc(\helperConfig,\poseBeliefSensor) 
= 
\mathbb{E}_{\objPose \sim \poseBeliefSensor}\left[{\graspScoreExpectation^{*}\left({\actorBeliefUpdate\left({\poseBeliefActor,\estimatedObservation_{\objPose, \helperConfig}}\right)}\right)}
-
{\graspScoreExpectation^{*}(\poseBeliefActor)}\right].
\end{equation}
\end{comment}
\end{definition}
%where $\predictedPoseBeliefGripper = \actorBeliefUpdate(\poseBeliefActor,\estimatedObservation_{\objPose, \helperConfig})$ is the updated belief the \actor~will have after receiving the predicated observation $\estimatedObservation_{\objPose, \helperConfig}$ of pose $\objPose$ from sensor configuration $\helperConfig$. 


\begin{comment}
%\begin{comment}
    
We chose an observation similarity metric
\begin{equation}\label{eq:obsScoreee}
\obsSimScore\left({\estimatedObservation_{\objPose,\helperConfig}, \observation_{\objPose,\helperConfig}}\right)
=
\frac{1}{\sigma\sqrt{2 \pi}}
e^{-\frac{1}{2}\left({\dfrac{\left\Vert{\estimatedObservation_{\objPose,\helperConfig} - \observation_{\objPose,\helperConfig}}\right\Vert}{\sigma}}\right)^{2}}.
\end{equation}
%\end{comment}

\dd{
\begin{equation}
\label{eq:graspVOA}
\VOAFunc(\helperConfig,\poseBeliefHelper) 
= 
\mathbb{E}_{\objPose \sim \poseBeliefHelper}\left[{\graspScoreExpectation^{*}\left({\predictedPoseBeliefGripper}\right)}\right]
-
{\graspScoreExpectation^{*}(\poseBeliefActor)}
\end{equation}
$$
=
\sum_{\objPose_i \in \allObjStablePoses}
\left[{
\poseBeliefHelper\left({\objPose_i}\right)
\sum_{\objPose_j \in \allObjStablePoses}
\left[{
\predictedPoseBeliefGripper\left({\objPose_j}\right)
\graspScoreFunc\left({
\argmax_{\graspConfig\in \graspConfigSet}
\left\lbrace{
\sum_{\objPose_k \in \allObjStablePoses}
\left[{
\predictedPoseBeliefGripper\left({\objPose_k}\right)
\graspScoreFunc\left({ \graspConfig, \objPose_k }\right)
}\right]
}\right\rbrace, \objPose_j }\right)
}\right]
}\right]
$$
$$
-
\sum_{\objPose \in \allObjStablePoses}
\left[{
\poseBeliefActor\left({\objPose}\right)
\graspScoreFunc\left({
\argmax_{\graspConfig\in \graspConfigSet}
\left\lbrace{
\sum_{\objPose \in \allObjStablePoses}
\left[{
\poseBeliefActor\left({\objPose}\right)
\graspScoreFunc\left({ \graspConfig, \objPose }\right)
}\right]
}\right\rbrace, \objPose 
}\right)
}\right]
$$
\begin{equation}
=
\sum_{\objPose_i \in \allObjStablePoses}
\left[{
\poseBeliefHelper\left({\objPose_i}\right)
\sum_{\objPose_j \in \allObjStablePoses}
\left[{
\predictedPoseBeliefGripper\left({\objPose_j}\right)
\graspScoreFunc\left({
\graspConfigMax, \objPose_j }\right)
}\right]
}\right]
-
{\graspScoreExpectation^{*}(\poseBeliefActor)}
\end{equation}
where
\begin{equation}
\predictedPoseBeliefGripper\left({\objPose_j}\right)
=
\dfrac{
\observationPerceivedProbability\left({\estimatedSensorFunc\left({\objPose_{i}, \helperConfig}\right) \vert \objPose_j, \helperConfig}\right)
\poseBeliefActor\left({\objPose_j}\right)
}{
\Sigma_{\objPose' \in \objStablePoses}
\observationPerceivedProbability\left({\estimatedSensorFunc\left({\objPose_{i}, \helperConfig}\right) \vert \objPose', \helperConfig}\right) \poseBeliefActor\left({\objPose'}\right)
}
\end{equation}
and
\begin{equation}
\graspConfigMax
=
\argmax_{\graspConfig\in \graspConfigSet}
\left\lbrace{
\sum_{\objPose_k \in \allObjStablePoses}
\left[{
\predictedPoseBeliefGripper\left({\objPose_k}\right)
\graspScoreFunc\left({ \graspConfig, \objPose_k }\right)
}\right]
}\right\rbrace.
\end{equation}
}
\end{comment}

\begin{algorithm}
\label{alg:chooseHelpAction}
\yuval{Note that this algorithm is correct for deterministic observation function, when it's stochastic we don't need $\estimatedSensorFunc$, we need $\observationPerceivedProbability$ instead. maybe write it after the algorithm?}
\SetKwFunction{MEAN}{Mean}
\SetKwFunction{SAMPLE}{Sample}
\SetKwFunction{COMPUTEVOA}{ComputeVOA}
\SetKwProg{FN}{Function}{:}{}
\caption{Choose helping action with \VOA}
\KwIn{Grasp configuration set $\graspConfigSet$}
\KwIn{Sampled subset of help configurations $\Tilde{\helperConfigs} \subseteq \helperConfigs$}
\KwIn{Actor belief $\poseBeliefActor$.}
\KwIn{Helper belief $\poseBeliefHelper$.}
\KwIn{Grasp score function $\graspScoreFunc$.}
\KwIn{Observation predication function $\estimatedSensorFunc$}
\KwIn{Sampled subset of object pose set $\tilde{\objStablePoses}\subseteq \objStablePoses$.}
\KwIn{Actor's belief update function $\actorBeliefUpdate$}
\KwOut{Sensor configuration $\helperConfig^{*} \in \Tilde{\helperConfigs}$}

Compute $\graspConfigMax(\poseBeliefActor)$; 
\Comment{Chosen grasp without help. Equation \ref{eq:graspConfigMax}}

Compute $\graspScoreExpectation(\graspConfigMax(\poseBeliefActor), \poseBeliefHelper)$; 
\Comment{Mean score without help. Eq. \ref{eq:graspScoreExpectation}}

$\helperConfig^{*} \gets Null$\; \Comment{Chosen helping action}

${\VOAFunc}^{*} \gets 0$\; \Comment{best \VOA}

\For{$\helperConfig \in \Tilde{\helperConfigs}$}
{
    $\VOAFunc_{\helperConfig} \gets \COMPUTEVOA(\helperConfig, \Tilde{\objStablePoses}, \graspScoreExpectation(\graspConfigMax(\poseBeliefActor), \poseBeliefHelper)
    , \poseBeliefActor, \poseBeliefHelper, \actorBeliefUpdate)$\;\\
    \If{$\VOAFunc_{\helperConfig} > {\VOAFunc}^{*}$}
    {
        ${\VOAFunc}^{*} \gets \VOAFunc_{\helperConfig}$\;\\
        $\helperConfig^{*} \gets \helperConfig$\;
    }
}
\Return $\helperConfig^{*}$\;\\


\FN{\COMPUTEVOA$(\helperConfig, \Tilde{\objStablePoses}, \graspScoreExpectation(\graspConfigMax(\poseBeliefActor), \poseBeliefHelper), \poseBeliefActor, \poseBeliefHelper, \actorBeliefUpdate)$}
{
$\mathbf{\Gamma_{\Tilde{\objStablePoses}}} \gets \emptyset$;
\Comment{Score per sampled pose after help}

\For{$\objPose \in \Tilde{\objStablePoses}$} 
{
    $\estimatedObservation \gets \estimatedSensorFunc\left({\objPose, \helperConfig}\right)$; \Comment{predicted observation for pose}
    
    $\predictedActorBelief \gets \beliefUpdateFunc\left({\poseBeliefActor, \estimatedObservation}\right)$;
    \Comment{Predicted belief. Eq. \ref{eq:belief update}}
    
    Compute $\graspConfigMax(\predictedActorBelief)$; 
    \Comment{Chosen grasp with help. Eq. \ref{eq:graspConfigMax}}
    
    Compute $\graspScoreExpectation(\graspConfigMax(\predictedActorBelief), \poseBeliefHelper)$; 
    \Comment{Mean score. Eq. \ref{eq:graspScoreExpectation}}
    
    $\mathbf{\Gamma_{\Tilde{\objStablePoses}}} \gets \mathbf{\Gamma_{\Tilde{\objStablePoses}}} \cup \{\graspScoreExpectation(\graspConfigMax(\predictedActorBelief), \poseBeliefHelper) \}$\;
}

\Return $\MEAN(\mathbf{\Gamma}_{\Tilde{\objStablePoses}}) - \graspScoreExpectation(\graspConfigMax(\poseBeliefActor))$\; \Comment{Eq. \ref{eq:generalVOAInf1}}
}
\textbf{end function}
\end{algorithm}

\todo{how VOA is used for selecting an sensor configuration}
Algorithm \ref{alg:chooseHelpAction} describes how a helper agent can choose a beneficial helping action by sampling a set of helping actions from $\helperConfigs$, using VOA to evaluate them and choosing the action with the greatest VOA. In the algorithm a subset of stable poses is sampled from the helper belief distribution, this subset of poses is used to approximate the expectation in equation \ref{eq:generalVOAInf1} for each of the sampled helping actions. 
The algorithm includes the implementation of the ComputeVOA function for a single helping action given the subset of sampled poses, the expected grasp score without intervention, and the beliefs of the actor and helper agents. Considering a single agent with both sensing and grasping capabilities, or two agents that share the same belief, the computation remains the same, with $\poseBeliefActor = \poseBeliefHelper$.

\subsection{Complexity Analysis}

Exploring the complexity of algorithms is vital, it allows us to understand how the algorithm's performance scales with the size of the input or other relevant parameters. Additionally, analyzing the complexity can lead to insights for optimization and improvement, making the algorithm more efficient. As we analyze the steps of our algorithm, we'll keep an eye out for any parts that seem too slow or complicated. If we find these spots, we might be able to make them better.% We'll carefully go through the algorithm, step by step, to figure out its complexity, with the hope of finding ideas that might help improve it later on.

    We observe that $\estimatedSensorFunc\left(\helperConfig,\objPose\right)$ could be a bottleneck in the algorithm, depending on the sensor used. We will denote its complexity as $O(\alpha)$.

    \begin{enumerate}
        \item Outer Loop Over $\allObjStablePoses$: The outer loop iterates over the set of poses $\allObjStablePoses$, so it runs $|\allObjStablePoses|$ times.
        \item Observation Prediction Function and Belief Update: Within each iteration of the outer loop, the alpha function is called, adding $O(\alpha)$. The belief update is also called, which contains its own internal loop over $\allObjStablePoses$ and calls the alpha function in each iteration. Therefore, the belief update contributes $|\allObjStablePoses| \times O(\alpha)$.
        \item Grasp Calculation Over $\graspConfigSet$ and $\allObjStablePoses$: The best grasp calculation, which occurs for each pose, has a complexity of $|\graspConfigSet||\allObjStablePoses|$ since it runs for each grasp configuration and each pose.
    \end{enumerate}

    Combining the complexities from these components, we get:

    \begin{itemize}
        \item For each pose in $\allObjStablePoses$, the alpha function and the belief update yield $O(\alpha) + |\allObjStablePoses| \times O(\alpha)$.
        \item The grasp calculation contributes $|\graspConfigSet||\allObjStablePoses|$.
    \end{itemize}

    So the total complexity is given by: $|\allObjStablePoses| \times \left(O(\alpha) + |\allObjStablePoses| \times O(\alpha) + |\graspConfigSet||\allObjStablePoses|\right)$.

    Simplifying this expression, we get: $$O\left(|\allObjStablePoses|^2|\graspConfigSet|\right) + O\left(|\allObjStablePoses|^2 \times \alpha \right)$$

    our algorithm is developed for a specific sensor configuration $\helperConfig$. When we extend the algorithm to perform an $arg \max$ operation over a set of possible sensor configurations $\helperConfigs$ the time complexity becomes $O\left(|\helperConfigs|\times\left(|\allObjStablePoses|^2|\graspConfigSet| +|\allObjStablePoses|^2 \times \alpha \right)\right)$

    One significant optimization we've introduced involves the computation of $\alpha$ values, which are utilized at least $|P_o|$ times within the algorithm. Recognizing this, we precalculate the entire set of $\alpha$ values upfront. This strategic approach reduces the overall complexity from $O(|\allObjStablePoses|^2 \times \alpha)$ to $O(|\allObjStablePoses| \times \alpha)$. Subsequently, whenever an $\alpha$ value is needed, it can be retrieved in constant time, $O(1)$, significantly streamlining the algorithm's execution. However, it's important to note that this approach requires additional memory to store the precomputed observations values, thereby increasing the algorithm's space complexity. The overall time complexity is now $O\left(|\allObjStablePoses|^2|\graspConfigSet|\right) + O\left(|\allObjStablePoses| \times \alpha \right)$.

%Importantly, the \helper~and \actor~may not have the same belief or belief update function. %We therefore distinguish here between the belief of the 
\sk{TODO}
\begin{comment}
    
\pagebreak
$$
=
\sum_{\objPose \in \allObjStablePoses}
\left[{
\poseBelief\left({\objPose}\right)
\graspScoreExpectation^{*}(\poseBelief')
}\right]
-
{\graspScoreExpectation^{*}(\poseBelief)}
$$
$$
=
\sum_{\objPose_i \in \allObjStablePoses}
\left[{
\poseBelief\left({\objPose_i}\right)
\sum_{\objPose_j \in \allObjStablePoses}
\left[{
\poseBelief'\left({\objPose_j}\right)
\graspScoreFunc\left({
\argmax_{\graspConfig\in \graspConfigSet}
\left\lbrace{
\sum_{\objPose_k \in \allObjStablePoses}
\left[{
\poseBelief'\left({\objPose_k}\right)
\graspScoreFunc\left({ \graspConfig, \objPose_k }\right)
}\right]
}\right\rbrace, \objPose_j }\right)
}\right]
}\right]
$$
$$
-
\sum_{\objPose \in \allObjStablePoses}
\left[{
\poseBelief\left({\objPose}\right)
\graspScoreFunc\left({
\argmax_{\graspConfig\in \graspConfigSet}
\left\lbrace{
\sum_{\objPose \in \allObjStablePoses}
\left[{
\poseBelief\left({\objPose}\right)
\graspScoreFunc\left({ \graspConfig, \objPose }\right)
}\right]
}\right\rbrace, \objPose 
}\right)
}\right]
$$
\end{comment}

\begin{comment}
\begin{equation}
=
\sum_{\objPose_i \in \allObjStablePoses}
\left[{
\poseBelief\left({\objPose_i}\right)
\sum_{\objPose_j \in \allObjStablePoses}
\left[{
\poseBelief'\left({\objPose_j}\right)
\graspScoreFunc\left({
\graspConfigMax_{\poseBelief'}, \objPose_j }\right)
}\right]
}\right]
-
{\graspScoreExpectation^{*}(\poseBelief)}
\end{equation}
where
\begin{equation}
\poseBelief'\left({\objPose_j}\right)
=
\dfrac{
\observationPerceivedProbability\left({\estimatedSensorFunc\left({\objPose_{i}, \helperConfig}\right) \vert \objPose_j, \helperConfig}\right)
\poseBelief\left({\objPose_j}\right)
}{
\Sigma_{\objPose' \in \objStablePoses}
\observationPerceivedProbability\left({\estimatedSensorFunc\left({\objPose_{i}, \helperConfig}\right) \vert \objPose', \helperConfig}\right) \poseBelief\left({\objPose'}\right)
}
\end{equation}
and
\begin{equation}
\graspConfigMax_{\poseBelief'}
=
\argmax_{\graspConfig\in \graspConfigSet}
\left\lbrace{
\sum_{\objPose_k \in \allObjStablePoses}
\left[{
\poseBelief'\left({\objPose_k}\right)
\graspScoreFunc\left({ \graspConfig, \objPose_k }\right)
}\right]
}\right\rbrace.
\end{equation}
\end{comment}

%In our example, if grasping the mug at the handle has the highest grasp score, it doesn't matter if the mug is right side up or upside down; what matters is the angle of the handle. %Thus, in the example depicted in Figure \ref{fig:example-grasp}, it is not important to distinguish between two poses in which the handle is  
%we don't care about the object pose per-se: we only care about the belief change that will affect the probability of successfully grasping the object. %\yuval{maybe the last sentence should have a seperate subsection? I think this is the most important part}

%\section{Approaches to Grasp Belief Update}

\begin{comment}
With this agenda in mind, we consider three task-specific ways to perform the belief update, which vary in the assumption that are made on the available information and about the sensor and in their computational complexity. By offering this range of approaches we aim to support various settings for which the best approaches should be chosen based for the specific application. 

%\begin{itemize}
%    \item 0,1
%    \item Normalized Similarity metric
%    \item KL divergence 
%\end{itemize}
In all settings, we aim to estimate offline $\transformedPoseBelief_{\objPose}$ for each possible observation action, i.e.. the probability the \actor~will associate with each pose after receiving an observation $\predicatedObs$. Since at the time of computation, the actual pose each not known, We compute this value for given each possible pose $\objPose$.  
\end{comment}

%\dd{Hopefully we will see that it doesn't matter which method we choose.}

\begin{comment}
\subsubsection{A deterministic measure}
The first measure we consider computes whether two observations are exactly the same, i.e.
\begin{equation}
\observationPerceivedProbability\left({ \estimatedSensorFunc\left({\objPose', \helperConfig}\right) \vert \objPose, \helperConfig}\right)
=
\left\lbrace{
\begin{array}{cc}
   1  & \estimatedSensorFunc\left({\objPose', \helperConfig}\right) = \estimatedSensorFunc\left({\objPose, \helperConfig}\right)\\
   0  & \estimatedSensorFunc\left({\objPose', \helperConfig}\right) \neq \estimatedSensorFunc\left({\objPose, \helperConfig}\right)
\end{array}
}\right.
\end{equation}

%\sk{this is not a probability function- we need to normalize this }

\subsubsection{Using a Similarity Metric}
As a second option, we can base our computation on a similarity metric between two observations.

% define distance function
\begin{definition}[Observation Similarity Metric]
Given two observations $\observation_i, \observation_j \in \observations$, an {\em observation similarity metric} $\obsSimScore:\observations\times\observations\mapsto %\mathbb{R}_{\geq0}$
[0,1]$
associates a similarity score $\obsSimScore(\observation_i, \observation_j)$ between two observations.
\end{definition}

%Here we assume that $\estimatedSensorFunc$ is deterministic and noiseless, such that the distance between two observations taken from the same sensor configurations (and the same sensing action) are the same and the distance between them is 0. 
%find a way to quantify how informative an observation is The observation that we get is
%$\observation_{\objPose,\sensingAction} = \estimatedSensorFunc\left({ \objPose, \sensingAction}\right)$
%The observation for object pose $\objPose'$ is
%$\observation_{\objPose',\sensingAction} = \estimatedSensorFunc\left({ \objPose', \sensingAction}\right)$


% \begin{equation}\label{eq:obsScore}
% \obsScore(\objPose_j,\estimatedObservation_{\objPose_i,\sensingAction})= \frac{1-\obsDisScore(\estimatedObservation_{\objPose_i,\sensingAction}, \estimatedObservation_{\objPose_j,\sensingAction})}{\sum_{\objPose \in \allObjStablePoses}\left(1-\obsDisScore(\estimatedObservation_{\objPose_i,\sensingAction}, \estimatedObservation_{\objPose,\sensingAction})\right)}
% \end{equation}


%compute the Baysian update


In our case,
\begin{equation}
\observationPerceivedProbability\left({ \estimatedSensorFunc\left({\objPose', \helperConfig}\right) \vert \objPose, \helperConfig}\right)
=
\obsSimScore\left({\estimatedSensorFunc\left({\objPose', \helperConfig}\right), \estimatedSensorFunc\left({\objPose, \helperConfig}\right)}\right).
\end{equation}
%where $\eta$ is a normalization factor to ensure that we have a valid distribution function.

\dd{END}

\subsubsection{Using parameterized distribution}
In some settings, uncertainty can approximated tightly with a compact parametric model (e.g., a Gaussian distribution). For example, it is common to assume that a sensor reading is a XXX. 

In such cases, we assume that $\observationPerceivedProbability\left({\observation \vert \objPose, \helperConfig}\right)$ is given explicitly.
Then, given an observation $\predicatedObs$ we can compute its probability given each of the possible poses. 
In such cases, the normalizing factor is the sum of all probabilities. The benefit over using the metric measure is that here we only have $|\allObjStablePoses|$ computations, as opposed to $|\allObjStablePoses|^2$ we would have when using a similarity metric. 



%To account for such settings, we assume that the observation 
%\[
%  X \sim \mathcal{N}(\mu,\,\sigma^{2})\,.
%\] 

%In other cases, such approximations are too crude and more complicated representations most be employed. Recent research has successfully led to a range of are computationally efficient probabilistic algorithms, for a range of hard robotics problems—many of which are described in depth in this book


%The above formulation is general and can be used to support various settings, including different observation-prediction and perceived observation probability functions than the ones described in this paper.
%In the settings we examine here, we want to choose a single sensing action for a single agent and a single initial belief $\poseBelief$.



%\VOA~can be computed by only considering the first element in the formula, i.e., 
%$\VOAFunc(\sensingAction,\poseBelief) 
%= \graspScoreExpectation^{*}(\poseBelief^{\sensingAction}) $.



%\todo{See if we nee this:
%Based on the definition above, an optimal grasp $\graspConfigMax$ is one that maxmizes 
%\begin{definition}[Optimal Grasp] 
%Given a pose belief $\poseBelief$ over the set of possible stable poses $\objStablePoses$ and a set of possible grasping configurations $\graspConfigSet$, the {\em optimal grasp} is defined as follows
%$$\graspConfigMax = \argmax_{\graspConfig\in %\graspConfigSet}%{\graspScoreExpectation(\graspConfig)}. $$
%\end{definition}
%}


%We are interested  in assessing the informative value of an observation.  For this, we need a way to quantify the difference between observations



\end{comment}


%Specifically, given the current agent's belief regarding the object's pose and a description of possible sensing actions that can be performed, we seek a heuristic measure that is inexpensive to compute and that can be used to choose a sensing action that maximizes the probability of a successful grasp. 
%\dd{Is it really a question of where and when to perform a sensing action or is it rather about assessing the value of performing a sensing action? When and where might be out of this paper's scope.
%How about:


%the probability of different poses of the object. 

%We start by presenting a general formulation of \VOA~for grasping using sensing actions. In the following sections, we present how this general idea can be instantiated to support a specific setting and how we examine it empirically.  

%\subsection{Problem Statement}
%In its simplest form, the update is performed by comparing the observation to each possible object configuration. This can be done by taking any observation and...
%\todo{How belief update happens in practice and how it affects the probability of a successful grasp}
%\subsection{Grasp Belief Update Estimation}
%different in that we need to focus our attention 
%and on identifying how an observation will affect the task of that agent, and its ability to grasp the object. 




The \VOA~measure we develop here is based on the assumption that the agent that is performing its grasping task is equipped with one such methodology, and our aim it to account for the agent's policy in finding the best observation to support a successful grasping, our work is also strongly related to manipulation planning.



\subsection{TEMP}
The set $\allHelperConfigs$ was built by selecting robot configurations that were then translated into camera positions. Each position was evaluated for its view quality and distance to a key point of interest, prioritizing those that offered clear views while being suitably close, leading to a refined set of choices for capturing observations. The heuristic formula combines a distance score, which evaluates the camera's proximity to the Point of Interest (PoI), and a visibility score, which assesses how centered the PoI is within the camera's field of view. The total score is the sum of these two components.

The distance component measures the Euclidean distance between the camera and the PoI: $D(q)=\|FK(q)_{pos}-\mathcal{P}_{PoI}\|$ ,where $FK(q)_{pos}$ represents the position part of the end-effector (camera) pose obtained from the forward kinematics of configuration $q$, and $\mathcal{P}_{PoI}$ is the position of the PoI. The visibility component ensures the PoI is centered within the camera's FoV. This can be quantified by projecting the PoI onto the camera's image plane and measuring its deviation from the center of the image: $V(q)=\frac{\|Proj_{im(q)}(PoI)-C_{im(q)}\|}{R_{ref}}$ where $Proj_{im(q)}(PoI)$ calculates the projection of the PoI onto the camera's image plane, $C_{im(q)}$ is the center point of the image, and $R_{ref}$ is a reference radius or distance within the image plane that represents the boundary of acceptability. The combined heuristic: $$H(q)=\left(1-\frac{D(q)}{D_{max}}\right)+V(q)$$ where $D_{max}$ is a maximum acceptable distance to normalize the distance component.

%Here, we are interested in assessing the effect an observation will have the pose belief.
%Therefore, since we assume a finite set of possible object poses, the computation is based on comparing the difference between an observation made for a given pose $\objPoseOne$ and observations made from the same sensor configuration for other poses $\objPoseTwo\in \objStablePoses$.
%However, most approaches are general and offer ways to reduce state ambiguity. 
%and offer ways to estimate the probability distribution over possible world states.
%Our belief update is  focused on the grasping task and on supporting the decision of which grasp to attempt. 
%Notably, it implicitly assumed that for a given pose and sensor configuration, the emitted sensor is the same, i.e., $\observationPerceivedProbability\left({\observation \vert \objPose, \helperConfig}\right)=1$.
 
%\subsubsection{Using a Similarity Metric}


%The similarity metric can be used to compare the probability of the emitted observation $\observation$ and its probability $\observationPerceivedProbability\left({\observation \vert \objPose', \helperConfig}\right)$ for the different poses, thus highlighting distinct observations for which the probabilities are different. %to the observation that would be emitted for $\objPose'$. 
%\begin{equation}
%=
%\obsSimScore\left({\sensorFunc\left({\objPose', \helperConfig}\right), \observation}\right)
%\end{equation}
%where $\eta$ is a normalization factor to ensure that we have a valid distribution function.

%\subsubsection{Using parameterized distribution}



%\begin{itemize}
    %\item The grasped object has a known shape. % defined as $\objShape = \langle d,d,d \rangle$, where ...
    %\item We let $\allObjStablePoses$ represent the (possibly infinite) set of possible stable poses of an object. We assume the actual object pose $\objStablePose$ is within some known and finite subset of  $\allObjStablePoses$, $\objStablePose\in \objStablePoses \subseteq\allObjStablePoses$.
    %\item In this work, we are focused on parallel grippers, that can close and open a  gripper.  A grasping action consisting of closing the gripper. 
   % \item The \actor~state is known. %(noise is negligible) 
    %\dd{noisy gripper is the same as noisy object belief, and both manifest in the success probability, so this point doesn't really matter.}
    %\item The \actor~can choose one configuration in its configuration space from which to attempt a grasp.
    %\item We assume a finite set of possible grasping poses is given as input. dd{redundant, already covered in the second bullet.}
   % \item grasp score
 %\end{itemize}

%Our focus here is on assessing the expected benefit of receiving an observation and on supporting the decision of which intervention to perform, i.e., on choosing the most helpful observation.
%Accounting for the optimization considerations of the \helper~is beyond scope, and is an interesting avenue for future work.
%We aim to assist the decision of selecting a sensing action that causes a partially informed \actor~to select a grasp configuration that maximizes the probability of success.


%\subsection{Computing Grasp Score}
%\label{sec:grasp-score} 
%We define a configuration of the \actor~as a valid configuration of its end-effector. 


==> content/related.tex <==


\section{Related Work}

\begin{itemize}
    \item \url{ https://arxiv.org/pdf/2209.10342.pdf}
\end{itemize}


%\url{https://people.csail.mit.edu/lpk/papers/pomdp-grasp-final.pdf}
%\url{https://ieeexplore.ieee.org/document/9216952}
\temp{
Robot grasping for automation must be robust to the inherent uncertainty in perception, control, and physical properties such as friction. Computing robust grasp points on a given object is even more challenging when there are constraints due to a task intended to be performed with the object, for example in assembly, packing, and/or tool use. To compute grasps that robustly achieve task requirements, we designed an intuitive user interface that takes an object mesh as input and displays it, allowing non-specialists to indicate “stay-out” zones by painting facets of the mesh and to indicate desired forces and torques by drawing vectors. The interface then sends this specification to our server which computes resulting grasps and send them back to the client where the resulting parallel-jaw grasp axes are displayed color-coded by robustness.
}

==> content/table_all_metrics_backup.tex <==
    
\begin{table}[h!]
\centering
\begin{adjustbox}{angle=0}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{|c|c|ccccc|}
\specialrule{.1em}{.1em}{.2em} % Set midrule width
& &  $\SCOREDIFF$ & $\SCOREDIFFEXP$ & $\BESTSCOREEXPRATIO$ & $\ADVENTAGE$ & $\CONFIDENCEDIFF$\\
\specialrule{.2em}{.1em}{.2em} % Set midrule width
\multirow{6}{*}{$HOLDER$} 
& $\beliefUpdateFunc_1$ &  0.19 & 0.04 & 0.23 & 0.23 & 0.1\\
& $\beliefUpdateFunc_2$  & 0.15 & 0.03 & 0.23 & 0.29 & 0.09\\
& $\beliefUpdateFunc_3$  & 0.2 & 0.09 & 0.26 & 0.28 & 0.17\\
& $\beliefUpdateFunc_4$ & 0.03 & 0.1 & 0.15 & 0.13 & 0.11\\
& $\beliefUpdateFunc_5$ & 0.0 & 0.02 & 0.0 & 0.0 & 0.02\\
& $\beliefUpdateFunc_6$ & 0.0 & 0.01 & 0.0 & 0.0 & 0.01\\
\specialrule{.2em}{0em}{0em} % Set bottom rule width
\multirow{6}{*}{$EXPO$}
& $\beliefUpdateFunc_1$ & 0.29 & 0.31 & 0.31 & 0.29 & 0.14\\
& $\beliefUpdateFunc_2$ & 0.29 & 0.31 & 0.31 & 0.29 & 0.12\\
& $\beliefUpdateFunc_3$ & 0.29 & 0.31 & 0.31 & 0.29 & 0.22\\
& $\beliefUpdateFunc_4$ & 0.04 & 0.04 & 0.37 & 0.29 & 0.16\\
& $\beliefUpdateFunc_5$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.03\\
& $\beliefUpdateFunc_6$ & -0.00 & -0.00 & 0.29 & 0.29 & -0.00\\
\specialrule{.2em}{0em}{0em} % Set bottom rule width
\multirow{6}{*}{$MOUSE$}
& $\beliefUpdateFunc_1$ & 0.00 & 0.01 & 0.06 & 0.04 & 0.00\\
& $\beliefUpdateFunc_2$ & 0.00 & 0.01 & 0.05 & 0.04 & 0.00\\
& $\beliefUpdateFunc_3$ & 0.00 & 0.01 & 0.07 & 0.00 & 0.07\\
& $\beliefUpdateFunc_4$ & {\bf 0.04} & 0.05 & 0.44 & {\bf 0.53} & 0.12\\
& $\beliefUpdateFunc_5$ & 0.00 & 0.01 & 0.00 & 0.00 & 0.04\\
& $\beliefUpdateFunc_6$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.01\\
\specialrule{.2em}{0em}{0em} % Set bottom rule width
\multirow{6}{*}{$CUP$}
& $\beliefUpdateFunc_1$ & 0.30 & 0.33 & 0.33 & 0.30 & 0.10\\
& $\beliefUpdateFunc_2$ & 0.30 & 0.33 & 0.33 & 0.41 & 0.07\\
& $\beliefUpdateFunc_3$ & 0.37 & 0.50 & 0.63 & 0.37 & 0.22\\
& $\beliefUpdateFunc_4$ & 0.24 & 0.03 & 0.38 & 0.27 & 0.04\\
& $\beliefUpdateFunc_5$ & 0.00 & -0.00 & 0.00 & 0.00 & 0.00\\
& $\beliefUpdateFunc_6$ & 0.00 & -0.00 & 0.00 & 0.00 & 0.00\\
\specialrule{.2em}{0em}{0em} % Set bottom rule width
\multirow{6}{*}{$FLASK$}
& $\beliefUpdateFunc_1$ & 0.25 & 0.25 & 0.25 & 0.25 & 0.12\\
& $\beliefUpdateFunc_2$ & 0.25 & 0.25 & 0.25 & 0.25 & 0.12\\
& $\beliefUpdateFunc_3$ & 0.25 & 0.25 & 0.25 & 0.25 & 0.20\\
& $\beliefUpdateFunc_4$ & 0.02 & 0.07 & 0.25 & 0.25 & 0.15\\
& $\beliefUpdateFunc_5$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.02\\
& $\beliefUpdateFunc_6$ & 0.00 & 0.00 & 0.00 & 0.00 & -0.00\\
\specialrule{.2em}{0em}{0em} % Set bottom rule width
\multirow{6}{*}{AVG}
& $\beliefUpdateFunc_1$ & 0.19 & 0.04 & 0.23 & 0.23 & 0.10\\
& $\beliefUpdateFunc_2$ & 0.19 & 0.03 & 0.23 & 0.29 & 0.09\\
& $\beliefUpdateFunc_3$ & 0.20 & 0.09 & 0.26 & 0.28 & 0.17\\
& $\beliefUpdateFunc_4$ & 0.08 & 0.11 & 0.22 & 0.34 & 0.11\\
& $\beliefUpdateFunc_5$ & 0.00 & 0.02 & 0.00 & 0.00 & 0.02\\
& $\beliefUpdateFunc_6$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\specialrule{.2em}{0em}{0em} % Set bottom rule width

\end{tabular}


==> content/ws-evaluation.tex <==

\begin{figure}[t]
    \centering \includegraphics[width=7cm]{images/voa-lab-setup-2.png}
    \caption{Lab setup.}
    \label{fig:lab-setup}
    % \vspace{-0.4cm}
\end{figure}

\section{\VOA~for a Parallel Gripper and Lidar Sensor - a Preliminary Empirical Evaluation}\label{sec:ourSystem}\label{sec: Empirical Evaluation}

The objective of our evaluation is to examine the ability of our proposed \VOA~measure to predict the effect interventions in the form of sensing actions will have on the ability of the \gripperAgent~to successfully grasp the object and on finding the best intervention for maximizing that probability. 


With this objective in mind, our evaluation is comprised of three parts. 
\begin{enumerate}
    \item {\bf Evaluating \graspScore:} measuring the success ratio of the \gripperAgent's attempts to grasp an object given object pose and grasp configuration.
    \item {\bf Evaluating \observationPrediction}: examine the ability of our \observationPrediction~to predict the observation generated by the sensor for a \SensorConfiguration~and 
    object pose pair.
    \item {\bf Assessing \VOA~}: compare our \VOA~measure to the \emph{Average Executed Cost Difference} (AECD) achieved in our experiments and which represents the empirical difference between the grasp success probability with and without assistance.

\end{enumerate}
% In the following we first xxx and then... 

%\subsection{Experimental Setting}

We performed our evaluation in both a simulated and a real-world setting.
%Our \gripperAgent~is a UR5e robotic arm\footnote{https://www.universal-robots.com/products/ur5-robot/} with a parallel jaw gripper. The \sensorAgent~is a equipped with a lidar sensor.
Figure \ref{fig:lab-setup} shows our lab setup.
The \gripperAgent~is a $6$-DOF robotic arm\footnote{https://www.universal-robots.com/products/ur5-robot/} with a parallel-jaw gripper\footnote{https://onrobot.com/en/products/2fg7}.
We programmed the \gripperAgent~to perform a set of grasp configurations $\graspConfigSet \subset \mathbb{R}^6$ to grasp a mug positioned on a table.
The \sensorAgent~is a mobile robot\footnote{https://www.turtlebot.com/turtlebot3/},
with a lidar\footnote{https://emanual.robotis.com/docs/en/platform/turtlebot3/appendix\_lds\_01/} mounted on its top.
Figure \ref{fig:example-grasp} shows the same setup in a MuJoCo \cite{6386109} simulated environment.
We simulated the lidar using the MuJoCo depth camera, taking only the row at the height of the simulated sensor.
The simulated parallel jaw gripper is a Robotiq 2F-85\footnote{https://robotiq.com/products/2f85-140-adaptive-robot-gripper}.

We describe the sensor configuration as its 2D coordinates on the plane parallel to the floor at the lidar's level, and the robot's yaw or orientation, $\sensorConfigs \subset \mathbb{R}^3$.
Given the \sensorAgent's configuration $\sensorConfig \in \sensorConfigs$ and the lidar's reading in the agent's local frame, we can transform the sensor's reading to an observation $\observation$ as a set of points on the plane in the global frame.
 
%Each configuration $\graspConfig\in \graspConfigSet$ is defined by a $6$D vector $\graspConfig = \langle \px, \py, \pz, \pRoll, \pPitch, \pYaw \rangle$, where $\px, \py, \pz$ are the $3$D position of the end effector, and the $\pRoll, \pPitch, \pYaw$ represent the Euler angles of the end effector.



%for which a valid configuration is defined by a tuple $<\lidarPose, \orientation>$ such that $\lidarPose = \langle \px, \py \rangle$ defines a 2D Cartesian point and $\orientation$ is the orientation of the robot.
%A Lidar $360$ Laser Distance Sensor is mounted on the \sensorAgent at height $\lidarHeight$ from the ground.
%An observation is represented as an array $\observation= {\mathbb{R}_{\geq 0}}^{360}$ of 360 floats, with a cell for each degree for which the value describes the distance the laser has traveled.
%Each reading can be converted to a 2D point, representing the surface the lazer has hit. This is done by multiplying the distance by the cosine and the sine of the angle. 

Finally, the object shape $\objShape = (\Verticies, \Faces)$ is represented as a mesh comprised of a set of vertices $\Verticies \subset \Reals^{3}$ and faces $\Faces \subseteq \Verticies\times\Verticies\times\Verticies$.
The object pose $\objPose \in \mathbb{R}^6$, defines a local frame for the shape.
Given an object with a known shape, we can generate an observation prediction $\estimatedSensorFunc$ by simulating a sensing action at a configuration defined by $\sensorConfig$ and $\objPose$ by tracing rays from the simulated sensor, and recording the first intersection of these rays with the object's faces.

For assessing the grasp score function
$\graspScoreFunc$, we adopt an empirical approach to effectively capture the real-world effects of influential factors. 

%\todo{provide a score for an observation, given a known pose - in terms of the difference in the object poses}

Given an object pose $\objPose$ and sensing action $\sensingAction$ we want to assess the significance of the estimated observation
$\estimatedObservation = \estimatedSensorFunc\left({\objPose, \sensingAction}\right)$.
Intuitively, the more distinct the observation is from observations that could be made for other object poses, the more informative it is.
For examining the fit between two observations $\observation$ and $\observation'$, we calculate the root mean square deviation, $\rmsd\left({\observation, \observation'}\right)$.   
Then the significance of $\estimatedObservation$ given pose $\objPose$ is assessed accordingly.
%to the average distance of $\esitmatedObservation$ from the observations that would have been produced given the other poses $\objPose'\in \objStablePoses$.

Having obtained an evaluation of the grasp score $\graspScoreFunc$, we can assess \VOA~by updating the beliefs $\poseBeliefUpdated$
given the initial belief $\poseBelief$ and the observation prediction $\estimatedSensorFunc\left({\pose, \sensingAction}\right)$, $\forall \pose \in \allPoses$.


%$\rmsd\left({\estimatedSensorFunc\left({\objPose', \sensingAction}\right),\observation}\right)$.
%\begin{equation}\label{eq:observation-score}
%\observationScore(\estimatedObservation, \objPose) = 
%\end{equation}

%\dd{Given a $p$, what is the difference from $f_s(p)$ to $f_s(p')$. High difference is good.}

%\todo{compute the informative value with regards to the grasp configuration}

%\todo{take into account the pose belief}


%\begin{equation}\label{iBeliefUpdateFunc}
%\frac{{\left( + \rmsd\left({\estimatedSensorFunc\left({\objPose, \sensingAction}\right),\observation}\right)\right)}^{-1}}{\mathbb{E}_{\objPose' \sim \poseBelief}\left[{\left(\varepsilon + \rmsd\left({\estimatedSensorFunc\left({\objPose', \sensingAction}\right),\observation}\right)\right)}^{-1}\right]}\poseBelief(\objPose),
%\end{equation}


%To update the belief, we used the following belief update function $\poseBeliefUpdated = \beliefUpdateFunc\left(\poseBelief,\estimatedSensorFunc\left({\objPose, \sensingAction}\right)\right)$, \begin{equation}\label{iBeliefUpdateFunc}
%\poseBeliefUpdated
%=
%\frac{{\left(\varepsilon + \rmsd\left({\estimatedSensorFunc\left({\objPose, \sensingAction}\right),\observation}\right)\right)}^{-1}}{\mathbb{E}_{\objPose' \sim \poseBelief}\left[{\left(\varepsilon + \rmsd\left({\estimatedSensorFunc\left({\objPose', \sensingAction}\right),\observation}\right)\right)}^{-1}\right]}\poseBelief(\objPose),
%\end{equation}
%where $\rmsd\left({\estimatedSensorFunc\left({\objPose, \sensingAction}\right),\observation}\right)$ is the root mean square deviation of the distances between the observation $\observation$ and an observation prediction given $\sensingAction$ from where the observation $\observation$ was captured and $\varepsilon$ is a small value inserted to prevent division by zero in case of an exact match.

% \mm{another way to define it: $\objShape = (\Verticies, \Faces)$, where $\Verticies \subset \Reals^{3}$ and $\Faces=\Verticies \times \Verticies \times \Verticies$}
%\end{definition}

\iffalse
How do we calculate the grasp score Q? Done.
How do we update the belief tau?
How do we generate an observation prediction f\_s? Done.
\fi


% each reading in $\observation$ converted to a $3D$ point and the object positioned at $\objPose$.

%The observation prediction function $\estimatedSensorFunc$ for our lidar is as follows: the shape of the object is known, so for a given pose we calculate the intersection of the shape and lidar's level plane. After that in a 2D plane we put the resulting contour in the right place and a point that represents the lidar. for each angle in the 360 angles we calculate the first intersection point between the line that pass through the lidar point at this angle and the contour. then the distance between this point and the lidar point is assigned to the angle.


% \begin{algorithm}
% \caption{\observationPrediction}
% \begin{algorithmic}[1]

% \State \textbf{Input}:
%    \State Object shape $\objShape = (\Verticies, \Faces)$
%    \State Object pose $\objPose = dsdsds$ 
%    \State Sensor configuration $\sensorConfig = \langle \lidarPose,\lidarHeight\rangle$ 
% \State \textbf{Output}: estimated observation $\estimatedObservation = {\mathbb{R}_{\geq 0}}^{360}$ %\textit{angle\_distances} array containing distances from LiDAR to the object.
% \State \textbf{Initialize}:
%    \State Define \textit{angles} as an array from 0 to 359 degrees in 1-degree increments
%    \State Initialize an empty array \textit{angle\_distances} to store distances

% \State
% \State Create \textit{object\_polygon} using \textit{object\_shape} and \textit{object\_pose}
% \State Calculate \textit{object\_contour} as the intersection of \textit{object\_polygon} and the x-y plane at height \textit{$l_h$}

% \For{\textbf{each} \textit{angle} \textbf{in} \textit{angles}}
%     \State Create \textit{angle\_line} as a \textit{LineString} from \textit{$l_p$} with slope tan(\textit{angle})
%     \State Calculate \textit{intersection\_point} as the intersection of \textit{angle\_line} and \textit{object\_contour}
%     \State Calculate \textit{distance} as the Euclidean distance between \textit{$l_p$} and \textit{intersection\_point}
%     \State Append \textit{distance} to \textit{angle\_distances} array
% \EndFor
% \State return \textit{angle\_distances}

% \end{algorithmic}
% \label{alg:obsPredict}
% \end{algorithm}

%Diverse factors may impact the grasp success. Such factors may be contact area, closure force, object shape, and friction coefficient. 
%By focusing on empirical observations rather than attempting to model the intricate interactions of all factors comprehensively, we prioritize a practical understanding of grasp success.

%The different elements of the system and the interface between them are described in Figure \ref{}.



%\begin{figure}[ht!]
%\includegraphics[width=0.8\textwidth]%{images/system-configuration.jpg}
%caption{ %\textbf{
%The different components of grasp \VOA~estimation. } 
%\label{fig:setup}
%\end{figure}


%\section{Accounting For Continuous Space Representations}

Figure \ref{fig:voa-heatmap} shows some of our preliminary results\footnote{Due to space constraints, we provide the full details of our evaluation at \url{https://github.com/CLAIR-LAB-TECHNION/GraspVOA}.} indicating our \VOA~measure can be used to predict optimal grasp configurations.
%This includes evaluation using the MuJoCo environment (depicted in Figure \ref{fig:example-grasp}) and our lab setting, depicted in Figure \ref{fig:lab-setup}. 


%In both cases, our setup includes a \gripperAgent~that needs to choose a single \graspConfiguration~from which to attempt to grasp and object, and a \sensorAgent~that needs to choose a \sensorConfiguration~which .

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/voa-heatmap.png}
    \caption{Assessing grasp \VOA. The change in the belief due to a sensing action caused a shift in the grasp scores, in a way that changed the optimal grasp to OI90 from TD90.}
    \label{fig:voa-heatmap}
\end{figure}
